Android App Feature Extraction: A review of approaches for malware and app similarity detection

This paper reviews work published between 2002 and 2022 in the fields of Android malware, clone, and similarity detection. It examines the data sources, tools, and features used in existing research and identifies the need for a comprehensive, cross-domain dataset to facilitate interdisciplinary collaboration and the exploitation of synergies between different research areas. Furthermore, it shows that many research papers do not publish the dataset or a description of how it was created, making it difficult to reproduce or compare the results. The paper highlights the necessity for a dataset that is accessible, well-documented, and suitable for a range of applications. Guidelines are provided for this purpose, along with a schematic method for creating the dataset.

==> Aenderungen/Tracking.tex <==
Kapitel 1 und 2 wurden zusammengelegt da

Rev 2: Bitte beachten Sie den folgenden Hinweis. Meiner Meinung nach enthält Abschnitt 2 zu viele technische Details zur Arbeit an der Umfrage. Ich hätte es auf ein paar Sätze geschrumpft und es mit der Einleitung verschmolzen. (So etwas wie „Wir haben XYZ-Suchmaschinen und ConnectedPapers verwendet, um die relevantesten referenzierten Artikel auszuwählen, die nach 2001 veröffentlicht wurden.“ + einige Argumente, warum dieser Ansatz sicherstellt, dass nichts Wichtiges fehlt.)

Kapitel 1 

Klärung der Forschungslücke:
Rev1: 1. Sie haben die Notwendigkeit erwähnt, gleichzeitig schädliche Apps zu erkennen und Lösungen bereitzustellen, die dieselben Daten verwenden. Sie haben es zwar aus Anwendersicht erklärt, können Sie aber auch näher erläutern, warum es aus Forschersicht in der vorhandenen Literatur an solchen Studien mangelt? Gibt es besondere Herausforderungen bei der Durchführung einer solchen Forschung?

und 

Aufnahme anderer Review paper wegen:
Rev 1: 2. Gibt es weitere relevante Umfragepapiere in diesem Bereich? Eine vergleichende Analyse verwandter Werke wäre wertvoll.

Kapitel 2:

Aufnahme Fußnote 2:
Kap 2.2
Rev 1: 4. In Abschnitt 3.2 haben Sie Probleme im Zusammenhang mit Datenquellen zum Sammeln von Android-Anwendungen erwähnt. Es bleibt jedoch unklar, wie Sie diese Herausforderungen angegangen sind, um die in Tabelle 2 aufgeführten Quellen zu erhalten.

Tabelle 2 update der quellen und extended version im apendix
Rev 1: 5. Es ist nicht ersichtlich, wie sich die extrahierten Merkmale zwischen verschiedenen Tools unterscheiden oder ob es zwischen ihnen Überschneidungen gibt. Erwägen Sie die Verwendung einer Tabelle, um die von diesen Tools extrahierten kritischen Funktionen zu skizzieren und zu erläutern, wie diese Funktionen zur Android-Anwendungsanalyse beitragen. Darüber hinaus wäre es hilfreich, die spezifische Funktionalität dieser Tools bei der Erkennung bösartiger oder ähnlicher Anwendungen zu erläutern.

Kapitel 4

Komplett überarbeitet wegen:
Rev 1: 7. Der Vorschlag zur Erstellung eines universellen interdisziplinären Datensatzes in Abschnitt 5 ist ein bemerkenswerter Beitrag. Eine klarere und detailliertere Beschreibung der Erstellung eines solchen Datensatzes oder die Gestaltung eines Rahmenwerks zur Lösung der Probleme würde das Papier bereichern.

Kapitel 5
Komplett überarbeitet wegen:
Rev 1: 8. In Abschnitt 6 erscheint die Analyse unzureichend und die Schlussfolgerung ist nicht aussagekräftig. Es wird empfohlen, bestehende Ansätze umfassend aus mehreren Perspektiven zu diskutieren, um diesen Abschnitt zu stärken.


==> sections/01_introduction/20240428_01_Introduction.tex <==
\section{INTRODUCTION}
\label{sec:intro}

Smartphones are becoming increasingly important and indispensable for people’s daily lives because they offer a range of convenient features and functions that simplify everyday tasks. However, this fact leads to a dependency between users and their smartphones which can be dangerous if compromised applications are used. 

According to Ericsson (cited by \cite{Turner.2023}), in 2021, 6.34 billion smartphones were in use. The most widespread smartphone operating system is Google's Android, with at least 71.45\% market coverage, followed by Apple's iOS, with about 27.83\% market coverage \cite{Statista.28.07.2022}. The popularity of Android also has its drawbacks. According to \citeauthor{Willems.2022}~\cite{Willems.2022} from GDATA, currently, more than 25 million malicious applications for Android have been detected. Furthermore, not only intentionally manipulated apps can harm users. Poorly programmed or outdated applications can also pose significant risks. According to atlasVPN \cite{Ruth.28.07.2022}, "63\% of Android applications had known security vulnerabilities in Q1 2021, with an average of 39 vulnerabilities per app", whereby gaming and finance apps have the most security issues. 

In addition, it is important to know how malware is commonly distributed. Piggybacking, also known as adding malicious code to pirated versions of popular apps, is a common method used to spread malware \cite{Zhou.2013}.\footnote{According to \citeauthor{Zhou.2012}~\cite{Zhou.2012}, pirated apps are not only used to inject malicious code; They can also be used to “replace existing in-app advertising or embed new ones to ‘steal’ or redirect advertising revenue.” In addition to the threat posed by pirated apps due to inserted malicious code, they also represent a violation of applicable copyright law.} Identifying nearly identical applications, especially those with subtle differences that may indicate the presence of malware, is critical to modern threat detection strategies.

Researchers have been grappling with these issues for the past decades, trying to identify dangerous and pirated applications, as well as detect similarities in apps. However, there is a lack of a holistic approach that addresses both the identification of risks, such as malware and clones, and the provision of (user-centric\footnote{Users may ignore risks and continue to use malicious applications if appropriate action options are not provided.}) options for action, such as providing harmless alternatives to dangerous applications. 
To fill this gap, requirements from both the scientific and the user perspectives was extracted from the literature. In addition, challenges related to the underlying data were derived that have negatively impacted the validation and replication of existing approaches in the past. Based on this, guidelines and requirements for a new dataset were formulated and a dataset generation system was designed.
%Researchers have been grappling with these issues for the past decades, trying to identify dangerous and pirated applications, as well as detect similarities in apps. However, there is a lack of a holistic and user-centered approach to risk mitigation like detecting hazards, providing actionable recommendations, and offering safe alternatives. After all, users can ignore risks and continue using malicious applications if adequate alternatives are not provided. This highlights the need to provide holistic solutions and is instrumental in strengthening users' digital sovereignty and helping non-technical users manage risk.

To ensure the development of such a holistic approach, the data set to be developed must ensure research in the following areas
%Three main areas of action can be derived to improve the situation for smartphone users and expand the scientific knowledge in the subject:

\begin{itemize}
\item First, systems need to be further developed to be able to detect malicious code in Android applications.
\item Second, systems must be researched and developed that show users safe alternatives and thus offer them recommendations for action by detecting functionally similar applications.
\item Third, combining the two previous domains can create new methods for detecting malicious applications, for example pirated and piggybacked apps\footnote{Detecting similar applications with minimal differences may indicate that they have been pirated or remarketed with malicious code \cite{Zhou.2013}.}. 
\end{itemize}

One difficulty in linking these domains is the lack of a current, extensive, and multipurpose dataset. Existing datasets are primarily related to malware detection and are often outdated\footnote{\label{MalwareDatasets}e.g. Android Genom Project \cite{Zhou.2012b}, M0DROID \cite{Damshenas.2015}, Drebin \cite{Arp.February23262014, Spreitzenbarth.2013}, Kharon \cite{Kiss.2016}, AAGM \cite{Lashkari.2017}, Android PRAGuard \cite{Maiorca.2015}, AndroZoo \cite{Allix.2016c}} or unavailable\footnote{e.g. ContagioDump, AndroMalShare, AMD Project}, making it difficult to compare, evaluate and reproduce research results in this area. Therefore, it is crucial to provide a comprehensive dataset that detects malware on the one hand and addresses user-centric risk mitigation systems on the other. In this study, we would like to address this issue and propose the creation of a dataset that supports the training of malware detection systems, the identification of cloned and possibly compromised applications, and the search for functionally similar but secure applications. 

To address this, we examine the literature on malware, app similarity, and clone detection published between 2002 and 2022 to identify all features suitable for creating such a dataset as well as the tools necessary to extract them. A keyword and snowballing search was performed to identify relevant literature\footnote{The keyword search was performed on "Google Scholar", "ACM digital library", and "IEEE Xplore" and included terms such as "Android + Similarity", "Clone + Android" and "Malware + Android". For the snowballing search, connectedpapers was used (https://www.connectedpapers.com/). This is a website to generate citation graphs based on the provided starting literature.}. %Altogether, over 5000 papers were inspected, and 286 were used for the analysis.

Furthermore, existing survey papers in the domains that have analyzed literature related to malware, app similarity, and clone detection were examined. However, these surveys often lack a comparative analysis between these domains, as well as a thorough discussion on the creation of derived datasets from identified features. For instance, \citeauthor{Li.2017}~\cite{Li.2017} focus on clone and malware detection but do not delve into similarity detection.\footnote{Contrary to the analysis in this paper, the authors analyze literature from 2011 to 2015.} \citeauthor{Firdaus.2018}~\cite{Firdaus.2018} explore static features extracted from app code and find the best feature set for malware detection by using a genetic algorithm but do not provide a comparative analysis of their application in clone and similarity detection. \citeauthor{Alzubaidi.2021}~\cite{Alzubaidi.2021} and \citeauthor{Feizollah.2015}~\cite{Feizollah.2015} also primarily concentrate on feature extraction for malware detection, neglecting similarity analysis. \citeauthor{Dhalaria.2021}~\cite{Dhalaria.2021} and \citeauthor{Jusoh.2021}~\cite{Jusoh.2021} provide detailed insights into malware detection techniques but do not discuss their results in the context of similarity detection. \citeauthor{Sharma.2021}~\cite{Sharma.2021} review 380 papers, offering a comprehensive overview of features and techniques but solely within the context of malware detection. \citeauthor{Selvaganapathy.2021}~\cite{Selvaganapathy.2021} also focuse on the area of malware detection. In their work, they provide a list of public datasets for malware detection and briefly discuss approaches to feature analysis and the tools most commonly used for this purpose.

Our research aims to address this gap by conducting a comprehensive literature mining process to identify features suitable for creating datasets for both similarity and clone detection as well as malware detection. Furthermore, we aim to explain the necessity for this dataset, the considerations to be taken into account during its creation, and the process of creating it. 

%In the coming chapters, this paper deals with a comprehensive analysis of Android applications and their extractable features and usage. In addition, the paper describes the creation of a universally applicable dataset and covers important aspects that are essential for the understanding and further development of this field.
%Through these chapters, this paper is intended to provide a holistic understanding of Android application analysis and, based on this, show how a universal dataset suitable for a wide range of different domains can be created to leverage synergies between these application domains and to make the research results more replicable and comparable.

%With this approach we ensured the inclusion of the most pertinent articles, guaranteeing a comprehensive overview of existing knowledge in the field\footnote{Statistics of analyze}. The remaining literature forms the foundation for analyzing features extractable from app stores and the Android Package (APK), as well as the tools to extract them, all of which are assessed according to their operational usability in various aspects of Android security. This approach not only facilitates the synthesis of existing research but also ensures that no crucial insights are overlooked.
 
%To address this gap, we employed a two-stage literature selection process to systematically identify and analyze relevant research spanning from 2002 to 2022. By utilizing a combination of different keywords and search engines, we ensured the inclusion of the most pertinent articles, guaranteeing a comprehensive overview of existing knowledge in the field. This methodological approach, combining both systematic and unsystematic strategies, facilitated the comprehensive identification of relevant literature within the specified timeframe.

%The aim of this paper is, therefore, to shed light on these challenges by providing an overview of tools and features used to detect Android security issues like malware or pirated copies as well as offering functionally identical and benign alternatives.

This paper is structured as follows: section 2 lays the technical foundations of Android application analysis and examines the mechanisms underlying these applications. In addition, sources for capturing applications are shown and tools that can be used to capture features are discussed. In section 3, different Android features extractable from the app stores or the APK files are introduced. It is also discussed how these features are used in different domains. Section 4 describes the process of generating a universal, interdisciplinary dataset, and forms the core of this work together with the analysis of extractable features. Section 5 critically discusses the limitations of this work. Finally, section 6 offers a reflection of the findings and implications from the previous chapters.



%The first section provides an overview of internal Android functionalities and tools to extract features. The second section presents features that can be mined from different sources like the Play Store or the internal APK. The final section summarises the results and discusses possibilities for future research. In particular, the easier comparability and reproducibility through the provision of a comprehensive dataset consisting of a wealth of Android features is discussed.

%Removed
%However, no dataset has yet been identified1 on which systems can be trained to recognize security-related vulnerabilities or provide options for risk reduction, such as suggesting substitute applications, let alone combining both fields. The datasets that do exist are often not published or not documented well. The material provided to replicate these datasets is not comprehensive. Therefore, comparing, evaluating, and reproducing research from the same field is difficult. 

%This paper will help close this gap by providing a review of tools and features used to detect Android security issues and providing functionally identical and harmless alternatives. The outcome of this review could be used to generate an interdisciplinary dataset connecting both fields. This dataset must fulfill the following requirements. First, detecting intentionally manipulated, poorly programmed, and outdated applications must be possible. Second, finding harmless applications providing similar features must also be possible. Third, the extracted features must be available before installing the application to analyze them before they can cause any damage. Fourth, the dataset must be publicly available, free to use, and well-documented. 



==> sections/02_Literatur_Selection_Process/02_Literatur_Selection_Process.tex <==
\section{LITERATURE SELECTION PROCESS}
\label{sec:literature_selection_process}

Finding relevant literature was limited by reducing the period and focusing on the topics of papers to investigate. The interval was limited to literature published between 2002 and 2022 because most research was published in this timeframe. The focus was set on literature covering the field of malware-, similarity- and clone detection because a system that should improve user security and digital sovereignty must cover all security-related fields as well as fields providing alternatives. Furthermore, the literature was filtered after reading the abstract, introduction, and conclusion. All literature pertaining to these areas was thoroughly reviewed.

The process of literature collection was done in two stages. First, an unsystematic approach to discovering relevant literature was performed. A combination of keywords like "Android + similarity", "clone + Android", and "malware + Android" were used on relevant literature search engines like "Google scholar", "ACM digital library", and "IEEE Xplore". The collected literature was filtered by the previously shown conditions. Second, this literature was used as a starting point for the second systematic paper collection stage. This stage was based on a snowballing process by collecting referenced papers. Therefore, the online tool connectedpapers\footnote{connectedpapers is a website to generate citation grapes based on the overhanded starting literature. It can be found under https://www.connectedpapers.com/.}  was used to draw reference graphs for all papers found in the previous stage. The resulting literature list was filtered by the same limiting conditions described above. Then all papers passing this process were likewise used as input literature for the snowballing mechanism. This process was repeated as long as no new relevant literature could be discovered.


==> sections/05_creating_universal_interdisciplinary_dataset/20240422_Backup.tex <==
\section{CREATING A UNIVERSAL, INTERDISCIPLINARY DATASET}
\label{sec:creating_universal_interdisciplinary_dataset}

%Android is the world's most widely used smartphone operating system \cite{Statista.28.07.2022} and represents a significant target for attackers. Therefore, it is crucial to provide a comprehensive data set that detects malware on the one hand and addresses user-centric risk mitigation systems on the other. This chapter defines the requirements that such a dataset must fulfill. This concerns both technical requirements for the data set and the consideration of the human factor as an important building block for risk mitigation. The process required to create such a data set is also described.

%Einleitung
As mentioned in the introduction a comprehensive data set that detects malware on the one hand and addresses user-centric risk mitigation strategies on the other is needed. This chapter defines the requirements that such a dataset must fulfill. This concerns both technical requirements for the data set and the consideration of the human factor as an important building block for risk mitigation. Furthermore, the process required to create such a data set is also described. But why is such a data set necessary?

%Notwendigkeit aus wissenschaftlicher Sicht
From a scientific point of view, the creation of a universal dataset enables a research environment that is easier to replicate and validate, facilitating the development of new methods and models. Furthermore, a universal dataset can be applied not only to specific use cases, but to a variety of other problems, leading to more general and robust solutions and enabling new domains of research. Furthermore, an existing data set significantly reduces the effort involved in data collection, as comprehensive data is already available. By consolidating all relevant features in one dataset, researchers can work more efficiently and at the same time exploit synergy effects between malware and similarity analysis. For instance, a system for detecting clones, provided that appropriate training data is available, could be expanded to detect subtle differences in these potentially identical applications. These discrepancies between applications may suggest the presence of malicious code within the app, potentially introduced through a process known as piggybacking\footnote{In piggybacking, an app is pirated and put back into circulation with malicious code\cite{Zhou.2013}}. A potential system based on subtle differences between apps was proposed by \citeauthor{Zhou.2013}~\cite{Zhou.2013}\footnote{Unfortunately, the authors do not make their data set publicly available.}. In addition, as demonstrated by \citeauthor{Zhou.2013}~\cite{Zhou.2013}, this approach can also be employed to automatically generate malware datasets by collecting and merging these discrepancies across multiple applications. The advantage of such similarity-and-difference-forming detection systems is that the malicious code does not have to be known beforehand, thus offering a way to detect unknown, malicious code fragments for further analysis\citeauthor{Zhou.2013}~\cite{Zhou.2013}. However, a comprehensive interdisciplinary data set is required for training and validation of such a system, as well as for research on systems to minimize risks for users of different behavioral levels. The creation of such a data set is therefore only possible through interdisciplinary research. Furthermore, interdisciplinary research opens up new possibilities by enabling collaboration and knowledge sharing between different research groups and disciplines. Ultimately, this also benefits users.

%Notwendigkeit aus nutzenden Sicht
In addition to the advantages to the research community, users will benefit from an enhanced level of security and user-friendliness in future systems. These systems will not only be able to detect malware but will also offer specific recommendations for action, such as alternatives to potentially dangerous applications\footnote{For example, \citeauthor{LinaresVasquez.2016}~\cite{LinaresVasquez.2016} have proposed a system for detecting similar Android applications, which could be used for this purpose.}. This is particularly important because user studies suggest that risk mitigation systems only achieve their full potential when the perceived cost of risk mitigation does not exceed the perceived effectiveness \cite{Alsaleh.2017, Hansen.2004, Liang.2009, Sasse.2005}. Different user groups must be addressed through adapted security mechanisms and options for action \cite{Hansen.2004,Sasse.2005}\footnote{Providing security-relevant information to technically-savvy users can overwhelm non-technically savvy users, which in turn represents a security risk for everyone.}. It would also be feasible to develop systems for proactive protection against threats. Furthermore, the detection of pirated software not only leads to a more secure environment but also improves the quality and integrity of the applications on offer. Moreover, the adaptation of systems addressing the individual needs of users enables an improved user experience for all user groups, regardless of their technical background.

% Zusammenfassung der Notwendigkeit
A significant barrier to the research, validation, and replication of all of these and also for future approaches are missing, unpublished, poorly documented or no longer available data sets\footnote{For example, the dataset referenced by \citeauthor{Schmicker.2019}~\cite{Schmicker.2019} is no longer available. The dataset used by \citeauthor{Sahs.2012}~\cite{Sahs.2012} is poorly documented, while \citeauthor{Shabtai.2010}~\cite{Shabtai.2010} offer only the data source without additional information. \citeauthor{LinaresVasquez.2016}~\cite{LinaresVasquez.2016} provide the application names and labels but not the extracted features.}. This highlights the need to create an interdisciplinary, universal, and freely available data set. The lack of suitable data not only makes comparability and reproducibility more difficult but also significantly hinders the research and further development of systems based on AI or AutoML. In addition, the development and evaluation of complex security systems for detecting malicious apps and providing options for action is hardly possible without appropriate data, as these systems usually require a large number of different features.  

This shows a considerable lack of universal data sets that are suitable for malware detection and at the same time take the human factor into account. Existing datasets show deficiencies in data quality, data acquisition, data storage, and dataset generation, with most deficiencies being due to reliability, timeliness, and availability. To address these issues, we have defined a set of requirements that must be met by and with future datasets. These requirements are not limited to the areas explained in this paper but can also be partially transferred to other domains.

\begin{itemize} 

\item{\textbf{Providing apps for different purposes:}} To recognize cloned applications or to detect minimal differences between the original and the pirated app, data records are required that contain the original apps, pirated copies, and derivatives with malicious code. To develop systems for providing options for action, a data set is required that shows similarity relationships between the applications using labels.

\item{\textbf{Providing multipurpose features and labels:}} Most existing data sets either only provide the app and the label or app features derived for a specific use case. However, to create a database for validation, replication, and further development of existing systems, the data set must have a wide variety of features and labels that are useful for different purposes. 

\item{\textbf{Research data management:}} Long-term, high-quality, cross-institutional data management is required to ensure availability and timeliness. To be able to react to current developments and validate previously published works with the same data set version, it is necessary to implement mechanisms that enable the data to be updated quickly and constantly. In order to ensure replication and verifiability, it is essential to guarantee that all dataset versions are permanently available.

\item{\textbf{Quality of the data sources:}} Future data sets must be based on knowledge from various sources to improve the reliability and completeness of the data sets and to prevent attempts at manipulation.

\item{\textbf{Documentation of used resources and vorgehen:}} schreiben unten in zusammenfassung schreiben das diese drei punkte wichtig sind für das replizieren

\end{itemize}

The generation of such datasets requires non-trivial feature extraction processes and the provision of suitable labels. Therefore, this article investigated which tools can be used and which features can be extracted from Android applications and their marketplaces to compile a comprehensive collection of features. These apps were also assigned corresponding labels by hand. This process can be improved in the future through a crowd-sourcing approach. The corresponding infrastructure has already been created. This data forms the basis for creating an interdisciplinary data set. To test its suitability, a system for generating an interdisciplinary data set and a system for evaluating app similarities was developed\footnote{It is currently still being clarified whether it is legally possible to publish the database, the data set generator, and the test system. The background is the copyright law in force in the EU, which prohibits crawling and analyzing copyrighted software}. The proposed extraction system uses a Selenium crawler to retrieve app APKs and useful information such as app name, size, developer, rating, version, description, categories, and required Android version from both the PlayStore and alternative sources. With the help of Androguard, data such as API calls\footnote{We extract all Android-specific, third-party-specific, and app-internal APIs and derive the package name, class name, function name, and frequency of the function call}, CallGraphs, strings, sensors, intentions, permissions, functions, activities, services, and recipients can be extracted from the app APK. In addition, all collected apps are scanned for viruses by VirusTotal. The scan result is also included as a feature in the data set. This data is used to train an autoencoder that recognizes app similarities. In the future, this system will be expanded to include functions for detecting malware such as "piggyback" malware through differential analysis.



==> sections/05_creating_universal_interdisciplinary_dataset/20240427_Backup.tex.tex <==
\section{CREATING A UNIVERSAL, INTERDISCIPLINARY DATASET}
\label{sec:creating_universal_interdisciplinary_dataset}

%Einleitung
After describing the data sources, extraction tools and features most often used to analyze research questions in similarity, clone and malware detection, this section.


As mentioned in the introduction, a comprehensive data set that detects malware on the one hand and addresses user-centric risk mitigation strategies on the other are needed. Before delving into the requirements and creation of such a dataset, it is important to recap the key takeaways from the previous sections. Section \ref{sec:technical_foundation} examined the technical foundations of Android application analysis, including the mechanisms underlying Android applications, strategies for capturing Android applications, and the technical foundations of feature extraction. It was shown that current research is difficult to validate and replicate due to various problems with the underlying dataset. Section \ref{sec:extractable_android_features} then focused on extractable Android features, discussing features that can be extracted from both app stores and APK files. It was shown that many features can be used across multiple areas of Android security, leading to potential synergies and symbiotic systems that can benefit from each other.

Building on these discussions, this section shifts its focus to defining the requirements for a comprehensive data set. First, the necessity for the creation of such a data set is presented from both the scientific and user perspectives. Based on this, the technical requirements for the data set are defined, and the human factor is examined as an important component of risk reduction. Finally, the schematic process required to create the data set is described.

%This section defines the requirements that such a dataset must fulfill. It begins by outlining the necessity for the creation of such a dataset from both a scientific and a user perspective. It then proceeds to examine the scientific and technical requirements for the data set, as well as the human factor as an important component for risk reduction. Based on these insights, requirements for such a dataset are defined. Finally, the schematic process required to create the dataset is described.

%Notwendigkeit aus wissenschaftlicher Sicht
From a scientific point of view, the creation of a universal dataset enables a research environment that is easier to validate and replicate, facilitating and accelerating the development of new methods and models. Furthermore, a universal dataset can be applied not only to specific use cases, but to a variety of other problems, leading to more general and robust solutions and enabling new fields of research. Additionally, an existing data set significantly reduces the effort involved in data collection, as comprehensive data is already available which can lead to results more quickly. By consolidating all relevant features in one dataset, researchers can work more efficiently and at the same time exploit synergy effects between malware and similarity analysis. For instance, a system for detecting clones, provided that appropriate training data is available, could be expanded to detect subtle differences in potentially identical applications. These discrepancies between applications may suggest the presence of malicious code within the app, potentially introduced through piggybacking \cite{Zhou.2013}. A potential system based on the detection of similarities and subtle differences between apps was proposed by \citeauthor{Zhou.2013}~\cite{Zhou.2013}\footnote{Unfortunately, the authors do not make their data set publicly available.}. The advantage of such a system is that the malicious code does not have to be known beforehand, thus offering a way to detect unknown, malicious code fragments for further analysis \citeauthor{Zhou.2013}~\cite{Zhou.2013}. A comprehensive interdisciplinary data set is required for training and validation of such a system, as well as for research on systems to minimize risks for users of different skill levels. The creation of such a data set is therefore only possible through interdisciplinary research. Furthermore, this type of research opens up new possibilities by enabling collaboration and knowledge sharing between different research groups and disciplines. Ultimately, this also benefits users.

%Notwendigkeit aus nutzenden Sicht
In addition to the advantages to the research community, users benefit from an enhanced level of security and user-friendliness in future systems. These systems are not only able to detect malware but also offer specific recommendations for action, such as alternatives to potentially dangerous applications\footnote{For example, \citeauthor{LinaresVasquez.2016}~\cite{LinaresVasquez.2016} proposed a system for detecting similar Android applications, which could be used for this purpose.}. This is particularly important because user studies suggest that risk mitigation systems only achieve their full potential when the perceived cost of risk mitigation does not exceed the perceived effectiveness \cite{Alsaleh.2017, Hansen.2004, Liang.2009, Sasse.2005}. Different user groups must be addressed through adapted security mechanisms and options for action \cite{Hansen.2004,Sasse.2005}\footnote{Providing security-relevant information to technically-savvy users can overwhelm non-technically savvy users, which in turn represents a security risk for everyone.}. It would also be feasible to develop systems for proactive protection against threats. Furthermore, the detection of pirated software not only leads to a more secure environment but also improves the quality and integrity of the applications on the market. Moreover, the adaptation of systems addressing the individual needs of users enables an improved user experience for all user groups, regardless of their technical background.

% Zusammenfassung der Notwendigkeit
A significant obstacle to the research, validation, and replication of current and future systems for protection against threats are unpublished, poorly documented, or no longer available data sets\footnote{As described in section \ref{ssec:gather_andorid_apps}, many authors do not provide clearly defined data collection methods or make datasets publicly available, hindering the replication and evaluation of proposed solutions. For example, the referenced dataset from \citeauthor{Zhou.2013}~\cite{Zhou.2013} is no longer available, and that from \citeauthor{Schmicker.2019}~\cite{Schmicker.2019} is no longer publicly accessible. The dataset used by \citeauthor{Sahs.2012}~\cite{Sahs.2012} is poorly documented, while \citeauthor{Shabtai.2010}~\cite{Shabtai.2010} offer statistical data without additional information about the underlying apps. \citeauthor{LinaresVasquez.2016}~\cite{LinaresVasquez.2016} provide a list of APK names and corresponding labels, but do not include necessary features like the application versions or the complete dataset with all extracted features.}. Existing datasets demonstrate deficiencies in data quality, data collection, data storage, and documentation. The majority of these deficiencies are due to a lack of reliability, timeliness, and availability. This scarcity of suitable data makes the comparability and reproducibility of studies more difficult. This issue is discussed by \citeauthor{Hutson.2018}~\cite{Hutson.2018}, who shows that AI is facing a reproduction crisis, as only about 6\% of authors publish their code and less than a third disclose their database. The absence of published code has negative effects on all areas of computer science, while the lack of available data sets is a particularly significant burden on research into modern AI systems. The unavailability of code and data, and the resulting issues with reproducibility greatly impede research progress. Furthermore, research reports often publish only a description of the data set generation process and not the actual data. Because of this, it is often not possible to reproduce the dataset due to inaccuracies and ambiguities in these descriptions. 

In addition, when analyzing the available datasets, it becomes apparent that researchers usually only extract the data that is relevant to their specific research. This makes a comparison with alternative approaches difficult, as those typically require different features. Another problem is the constant change and further development of the extraction tools on the one hand and the apps on the other, which leads to inconsistent replications. The lack of a standardized data set for evaluating the effectiveness of systems therefore leads to inconsistent results and makes it difficult to compare different approaches. Furthermore, the development and evaluation of complex security systems for detecting malicious apps and providing options for action is hardly possible without an adequate database, as these systems usually require a large number of different features. To address these challenges, we have defined a series of requirements that must be met by future data sets. These requirements extend beyond the domains discussed in this article and can be applied to other fields as well.

\begin{itemize} 

\item{\textbf{Providing apps for different purposes:}} To identify malicious and cloned applications, or to detect minimal differences between the original and the pirated application, data sets are needed that contain the original applications, malicious applications, and pirated copies with malicious code. Developing systems that provide options for action requires datasets with features that enable the identification of similarity relationships between applications.

\item{\textbf{Providing multipurpose features and labels:}} To create a database for validation, replication, and further development of existing systems, the data set must have a wide variety of features and labels that are useful for different purposes. Most existing data sets either only provide the app and the label or app features derived for a specific use case. These need to be expanded.

\item{\textbf{Research data management:}} Long-term, high-quality, and cross-institutional data management is required to ensure availability and timeliness. To be able to react to current developments and validate previously published works with the same data set version, it is necessary to implement mechanisms that enable the data to be updated quickly and constantly. In order to ensure verifiability and make replication possible, it is essential to guarantee that all dataset versions are permanently available. 

\item{\textbf{Quality of the data sources:}} Future data sets must be based on knowledge from several sources like different app stores and malware sources to improve their reliability and completeness and to prevent attempts at manipulation.

\item{\textbf{Documentation}}
A continuous and conscientious documentation of all work processes including the data collection, data preprocessing and data usage is essential.


\end{itemize}

Generating such datasets requires a non-trivial feature extraction procedure. The following is an example of how an effective tool chain could be structured based on the tools and features identified in this article. At the beginning of such a system is the collection of APKs. All sources mentioned in this article should be used. In addition to the APK, features such as app name, size, developer, rating, version, description, and app categories can be derived from the app stores. Existing databases such as the Android Genome Project (see \cref{tab:Tab_2_Android_APK_Sources}) should also be used. Web scrapers and crawlers can be used for this purpose.\footnote{See, for example, Selenium \cite{Selenium.20240423}, which can be used to automatically extract data from websites.}. The data should then be prepared and harmonized. For example, APKs downloaded from app stores should be analyzed with a virus scanner so that this data can be tagged with appropriate malware labels. On the other hand, the data from the existing datasets should be enriched with missing information, such as metadata from the app stores. A comprehensive dataset can then be generated from features such as API calls, call graphs, strings, sensors, intents, permissions, functions, activities, services, and recipients. It is advisable to use different tools and combine their results to get a better end result. The generated dataset should be usable for training malware and similarity detection systems.


==> sections/07_conclusion/07_conclusion_SH.tex <==
\section{CONCLUSION}
\label{sec:conclusion}

%According to \citeauthor{Feizollah.2015}~\cite{Feizollah.2015}, feature selection is a crucial first step in machine learning methods. 
This article analyzes the literature on Android malware detection, clone detection, and functional similarity detection between 2002 and 2022, with a particular focus on the data basis of features to be extracted for these systems. The work also examines the symbiotic relationship between these areas and how they can benefit from each other. Malware detection systems can benefit from clone detection systems because cloned applications often contain malicious code. Clone detection systems, in turn, can benefit from technical concepts of (functional) similarity detection systems, which in turn provide solutions for problems identified by malware and clone detection systems. The article also highlights the importance of having systems that provide options for action to mitigate security risks. Inexperienced users may not act appropriately despite warnings from malware or clone detection systems, which poses a potential risk to the entire Android ecosystem. Therefore, it is essential to have combined systems that inform users about dangerous applications and offer them options to protect themselves.

To achieve this objective, we extracted and analyzed fundamental data sources and tools for gathering information from multiple research reports. Furthermore, we examined valuable features that can be obtained from data sources, including the APK and various Android marketplaces, to establish the groundwork for such an integrated system. 

Features can be obtained from the official Google Play Store and secondary Android marketplaces from third-party providers, as well as from a limited number of public data sets in the area of malware detection. To extract features, we analyzed several tools and toolchains, including those for decompiling and analyzing the APK, examining the underlying Java code, and generating statistics and graphs. 

We also explored how extracted features can be made usable. In this analysis, we discuss existing approaches to feature extraction and their use from the malware, clone, and similarity detection perspective. Our goal is to gain deep insights into feature exploitation and uncover synergies. 

The evaluation of the information retrieval process showed that there is a wide range of methods and tools available for analysis. While textual features such as the app description, author information, or the app rating can be obtained by simply crawling the Android marketplaces, technical features extracted from the APK are often more reliable for security-relevant analyses due to their direct reference to the app functionality but are also considerably more complex to extract. Another advantage is, that this information cannot be manipulated or can only be manipulated with great effort in contrast to the marketplaces where developers sometimes manipulate data to achieve higher download rates \citeauthor{Pandita.2002}~\cite{Pandita.2002}. The most commonly used features of the APK are API calls, permissions, and code analysis. Since code is at the heart of any application, techniques such as extracting and analyzing diagrams, n-grams, and statistics, or using hashing and filtering techniques to reduce the search space have been extensively explored in this article. Metadata such as the internal structure of the application and textual features such as strings are used less frequently and treated in less detail.

Additionally, our analysis highlights the pressing need for publicly accessible databases of Android features across various research domains. Our analysis reveals a significant dearth of publicly accessible, universal, and interdisciplinary datasets. This lack of datasets impedes progress and collaboration in the field of Android security research. Therefore, this thesis also explores how to create such a dataset. This first step by analyzing the features found in the reviewed literature and the tools used to capture them. Afterward, we sketch a system for deriving such a dataset and explain how to compile a publicly available dataset for a wide range of Android security research. It is shown that synergies can be realized by extracting overlapping features between malware, clones and similarity detection.

Furthermore, significant challenges have been identified in the existing literature regarding data availability and reproducibility. Many authors do not provide clearly defined data collection methods or make datasets publicly available, hindering the replication and evaluation of proposed solutions. For instance, \citeauthor{LinaresVasquez.2016}~\cite{LinaresVasquez.2016} provide a list of APK names and corresponding labels, but do not include necessary features like the application versions nor the complete dataset with all extracted features. This issue is also discussed by \citeauthor{Hutson.2018}~\cite{Hutson.2018}, who shows that AI is facing a reproduction crisis, as only about 6\% of authors publish their code and less than a third disclose their database. The absence of published code has negative effects on all areas of computer science. However, the lack of available data sets is a particularly significant burden on research into modern AI systems. The unavailability of code and data, and the resulting issues with reproducibility, greatly impede research progress.

%To reduce the lack of data, one solution is to provide a universal and publicly accessible dataset that authors from different fields can reference.
To address the problem of reproducibility, journals should require a reference to a publicly accessible dataset or the publication of the dataset used, along with the publication of documentation and source code on the journal's website alongside the papers. This would enhance reproducibility and enable the broader research community to assess the findings of the published work.

The review not only summarizes the current state of research but also underscores the importance of collaborative efforts to overcome existing challenges. By promoting open data-sharing practices and encouraging reproducible research, we can promote the progress of Android security research and empower users to make informed decisions about app security.


% hier her verlegen aus Datensatz Kapitel
When analyzing the available datasets, it becomes apparent that researchers usually only extract the data that is relevant to their specific research, which makes a comparison with alternative approaches difficult, as these typically require different characteristics. Furthermore, it is common practice to publish only a description of the dataset generation process in the research report. In many cases, however, it is not possible to reproduce the dataset due to inaccuracies and ambiguities in the description. Another problem is the constant change and further development of the extraction tools on the one hand and the apps on the other, which leads to inconsistent replications. The lack of a standardized data set for evaluating the effectiveness of systems therefore leads to inconsistent results and makes it difficult to compare different approaches.

Another factor that should not be neglected is the quality of the data source on which the data set is based. Although data that can be accessed via Android marketplaces is easier to obtain than data that has to be extracted from the apps, it can also be manipulated more easily\footnote{Research by \citeauthor{Pandita.2002}~\cite{Pandita.2002} suggests that authors manipulate this data to achieve higher downloads}. \cite{Pandita.2002}. 

The generation of such datasets requires non-trivial feature extraction processes and the provision of suitable labels. Therefore, this article investigated which tools can be used and which features can be extracted from Android applications and their marketplaces to compile a comprehensive collection of features. 

==> sections/07_conclusion/07_conclusion_old.tex <==
\section{CONCLUSION}
\label{sec:conclusion}

According to \citeauthor{Feizollah.2015}~\cite{Feizollah.2015}, "in machine learning methods, feature selection is one of the first and most crucial steps". This paper reviewed the literature between 2002 and 2022 related to Android malware detection, (functional) similarity detection, and clone detection to filter out every useful feature. Additionally, the need for a combined system informing users of dangerous applications and providing them with courses of action to protect themselves was addressed. First, fundamental data sources and tools to extract information were presented. Second, features extractable from the APK and Android marketplaces were investigated to lay the foundations for such a system.

This paper evaluated which sources are available to collect information about Android APKs and malware. The official Google Play Store and 3rd party Android stores can be used to gather APKs. Different types of malware can be collected from datasets, most of which are publicly available. Several tools and toolchains were presented to examine Android applications: tools to decompile and analyze the APK, tools to investigate the underlying java code, tools to process the features like hash tools or graph generators, and tools that combine several others.

This paper explored features extractable from Android marketplaces and the APK. The most used features from Android marketplaces are textual features like the App description and metadata like author information or the app rating. Technical features crawled from Android marketplaces are used less frequently because they can also be mined from the APK in better quality. Furthermore, features mined from the APK are more reliable because authors can manipulate information in Android marketplaces to reach higher downloads \cite{Pandita.2002}. The most heavily used features mined by the APK are technical features like API calls, permission usage, and the application's code. Because the application's code is the heart of each application, this feature is examined in more detail. Therefore, this paper investigates several code analysis techniques like extracting graphs and n-grams, using statistics or using hashing and filtering techniques to reduce search space. On the other hand, metadata, like the app's inner structure and textual features like strings, are seldom used.

Finally, this paper has highlighted the lack of publicly available Android feature databases in the considered fields. It was found that no publicly available, universal, and interdisciplinary databases exist across these research areas. This review answers why such a dataset is helpful and how it can be constructed. Therefore, features found in the reviewed literature and the tools to collect them were outlined to compile a publicly accessible dataset useable for a wide range of Android security-related research. It was shown that the features extracted for Android malware and app similarity detection are applicable across most Android security-related fields.

Furthermore, this review has identified that many authors do not provide well-defined data collection methods, do not make their datasets publicly accessible, or provide inadequate documentation, making it difficult to replicate the proposed solutions and evaluate their effectiveness. For example, even the most exhaustive system by \citeauthor{LinaresVasquez.2016}~\cite{LinaresVasquez.2016} only provides a list of APK names and the corresponding labels but not the versions of the applications or a dataset including the extracted features. This problem was also described by \citeauthor{Hutson.2018}~\cite{Hutson.2018}, who states that AI is in a reproduction crisis because only about one in seventeen authors publishes their code, and less than a third publish their database. While the central issue in the general field of AI is missing code, data availability is also a fundamental concern for app similarity detection. This lack of data availability and reproducibility hinders the advancement of research. A solution to mitigate the lack of data is to provide a universal and publicly accessible dataset that authors in a wide range of fields can reference. To tackle the issue of reproducibility, it would be necessary for journals to require a reference to a publicly accessible dataset or the publication of the used dataset as well as the publication of documentation and source code on the journal's website alongside the writings. This would facilitate replicability and enable the wider research community to evaluate the outcomes of the published work.

